RIS-Assisted Interference Mitigation for Uplink NOMA

Non-orthogonal multiple access (NOMA) has become a promising technology for next-generation wireless communications systems due to its capability to provide access for multiple users on the same resource. In this paper, we consider an uplink power-domain NOMA system aided by a reconfigurable intelligent surface (RIS) in the presence of a jammer that aims to maximize its interference on the base station (BS) uplink receiver. We consider two kinds of RISs, a regular RIS whose elements can only change the phase of the incoming wave, and an RIS whose elements can also attenuate the incoming wave. Our aim is to minimize the total power transmitted by the user terminals under quality-of-service constraints by controlling both the propagation from the users and the jammer to the BS with help of the RIS. The resulting objective function and constraints are both non-linear and non-convex, so we address this problem using numerical optimization. Our numerical results show that the RIS can help to dramatically reduce the per user required transmit power in an interference-limited scenario.

==> arraymac.tex <==
% general purpose macros fo use with LaTeX (or TeX)
\makeatletter
\newfont{\sqi}{cmssqi8}
\newcommand{\IR}{\mbox{$I\!\!R$}}
\newcommand{\IC}{\mbox{$C\!\!\!\!\raisebox{.75pt}{\mbox{\sqi I}}\;\,$}}
\def\defnas{\stackrel{\rm def}{=}}
\newcommand\vdashl{\vdshl{1}{1}}
\newcommand\bvdashl{\vdshl{1.6}{2}}
\newlength{\tmpln}
\newlength{\dshln}
\newcommand{\vdshl}[2]{{\setbox1=\hbox{$[$}\setlength{\tmpln}{#1\ht1}
\advance\tmpln by #1\dp1
\setlength{\dshln}{.111\tmpln}
\newcommand\vs{\vskip .111\tmpln plus 1pt minus 1pt}
\newcommand\vd{\hrule width .4pt height \dshln depth 0pt}
\setbox2=\hbox{
 \vbox to\tmpln{\lineskip 0pt \lineskiplimit-1000pt \baselineskip 0pt
 \vd\vs\vd\vs\vd\vs\vd\vs\vd\vfil}$\;$}
 \lower#2\dp1\copy2
}}
\newcommand\adots{\mathinner{\mskip0mu\raise0pt\vbox{\kern7pt\hbox{.}}\mskip3mu
    \raise4pt\hbox{.}\mskip3mu\raise8pt\hbox{.}\mskip0mu}}
\def\nonumfootnotetext{\xdef \@thefnmark{}\@footnotetext}
\def\ie{{\it i.e.,\ }}
\def\cf{{\it cf.\ }}
\def\etc{{\it etc.}}
\def\etal{{\it et al.}}
\def\eg{{\it e.g.,\ }}
\def\apriori{{\it a~priori}}
\def\qed{%
   {%
      \unskip
      \nobreak \hfil
      \penalty 50               % TeX should break here if necessary
      \hskip 3em                % mimium amount of distance
      \null \nobreak \hfil
      \qedbox
      \parfillskip=\z@skip
      \finalhyphendemerits=\z@  % no line break at last line of paragraph
      \endgraf                  % don't know what \par is in this moment...
   }}
\def\qedbox{\rule[-1pt]{8pt}{8pt}}\def\QED{\qed}
%\def\beq{\@ifnextchar [{\@tempswatrue\@beq}{\@tempswafalse\@beq[]}}
%\def\@beq[#1]{\begin{equation}\edef\@tmparg{#1}\ifx\@tmparg\@empty \else
%        \label{#1}\fi}
\def\beq[#1]{\begin{equation} \label{#1}}
\newcommand{\eeq}{\end{equation}}
%\def\eeq{\end{equation}}
% \jot 2ex
\newcount\@eqcnt
\newcount\@eqpen
\newif\if@eqnsw\@eqnswtrue
\def\eqnarray{\stepcounter{equation}\let\@currentlabel=\theequation
\global\@eqnswtrue
\global\@eqcnt\z@\tabskip\@centering\let\\=\@eqncr
$$\halign to \displaywidth\bgroup\@eqnsel\hskip\@centering
  $\displaystyle\tabskip\z@{##}$&\global\@eqcnt\@ne
  \hskip .6\arraycolsep \hfil${##}$\hfil
  &\global\@eqcnt\tw@ \hskip .6\arraycolsep $\displaystyle\tabskip\z@{##}$\hfil
   \tabskip\@centering&\llap{##}\tabskip\z@\cr}
\def\str{\rule[-.6em]{0pt}{2.4em}}
\def\proof{\noindent {\bf Proof:\ }}
\let\pbox=\qed
\def\dag{{\cal y}}
\def\phstar{{\phantom{*}}}
\def\dmax{d_{\rm max}}
\def\vcv{\vdashl\cdots\vdashl}
\def\alphabf{{\boldsymbol \alpha}}
\def\betabf{{\boldsymbol \beta}}
\def\gammabf{{\boldsymbol \gamma}}
\def\deltabf{{\boldsymbol \delta}}
\def\epsilonbf{{\boldsymbol \epsilon}}
\def\epsbf{{\boldsymbol \epsilon}}
\def\zetabf{{\boldsymbol \zeta}}
\def\etabf{{\boldsymbol \eta}}
\def\thetabf{{\boldsymbol \theta}}
\def\iotabf{{\boldsymbol \iota}}
\def\kappabf{{\boldsymbol \kappa}}
\def\lambdabf{{\boldsymbol \lambda}}
\def\mubf{{\boldsymbol \mu}}
\def\nubf{{\boldsymbol \nu}}
\def\xibf{{\boldsymbol \xi}}
\def\pibf{{\boldsymbol \pi}}
\def\varphibf{{\boldsymbol \varphi}}
\def\rhobf{{\boldsymbol \rho}}
\def\sigmabf{{\boldsymbol \sigma}}
\def\taubf{{\boldsymbol \tau}}
\def\taubfh{\hat{\taubf}}
\def\upsilonbf{{\boldsymbol \upsilon}}
\def\phibf{{\boldsymbol \phi}}
\def\chibf{{\boldsymbol \chi}}
\def\psibf{{\boldsymbol \psi}}
\def\omegabf{{\boldsymbol \omega}}
\def\Gammabf{{\boldsymbol \Gamma}}
\def\Thetabf{{\boldsymbol \Theta}}
\def\Lambdabf{{\boldsymbol \Lambda}}
\def\Xibf{{\boldsymbol \Xi}}
\def\Pibf{{\boldsymbol \Pi}}
\def\Sigmabf{{\boldsymbol \Sigma}}
\def\Upsilonbf{{\boldsymbol \Upsilon}}
\def\Phibf{{\boldsymbol \Phi}}
\def\Psibf{{\boldsymbol \Psi}}
\def\Psibar{{\bar{\Psibf}}}
\def\Ebar{{\bar{\Ebf}}}
\def\Omegabf{{\boldsymbol \Omega}}
\def\Deltabf{{\boldsymbol \Delta}}
\def\abf{{\bf a}}
\def\bbf{{\bf b}}
\def\cbf{{\bf c}}
\def\dbf{{\bf d}}
\def\ebf{{\bf e}}
\def\fbf{{\bf f}}
\def\gbf{{\bf g}}
\def\hbf{{\bf h}}
\def\ibf{{\bf i}}
\def\iibf{{\bf ii}}
\def\iiibf{{\bf iii}}
\def\jbf{{\bf j}}
\def\kbf{{\bf k}}
\def\lbf{{\bf l}}
\def\ellbf{{\bf \ell}}
\def\mbf{{\bf m}}
\def\nbf{{\bf n}}
\def\obf{{\bf o}}
\def\peebf{{\bf p}}
\def\qbf{{\bf q}}
\def\rbf{{\bf r}}
\def\sbf{{\bf s}}
\def\tbf{{\bf t}}
\def\ubf{{\bf u}}
\def\vbf{{\bf v}}
\def\wbf{{\bf w}}
\def\xbf{{\bf x}}
\def\ybf{{\bf y}}
\def\zbf{{\bf z}}
\def\rbf{{\bf r}}
\def\xbf{{\bf x}}
\def\ybf{{\bf y}}
\def\Abf{{\bf A}}
\def\Bbf{{\bf B}}
\def\Cbf{{\bf C}}
\def\Dbf{{\bf D}}
\def\Ebf{{\bf E}}
\def\Fbf{{\bf F}}
\def\Gbf{{\bf G}}
\def\Hbf{{\bf H}}
\def\Ibf{{\bf I}}
\def\Jbf{{\bf J}}
\def\Kbf{{\bf K}}
\def\Lbf{{\bf L}}
\def\Mbf{{\bf M}}
\def\Nbf{{\bf N}}
\def\Obf{{\bf O}}
\def\Pbf{{\bf P}}
\def\Qbf{{\bf Q}}
\def\Rbf{{\bf R}}
\def\Sbf{{\bf S}}
\def\Tbf{{\bf T}}
\def\Ubf{{\bf U}}
\def\Vbf{{\bf V}}
\def\Wbf{{\bf W}}
\def\Xbf{{\bf X}}
\def\Ybf{{\bf Y}}
\def\Zbf{{\bf Z}}
\def\sf{\mathsf}
\def\asf{{\sf a}}
\def\bsf{{\sf b}}
\def\csf{{\sf c}}
\def\dsf{{\sf d}}
\def\esf{{\sf e}}
\def\fsf{{\sf f}}
\def\gsf{{\sf g}}
\def\hsf{{\sf h}}
\def\isf{{\sf i}}
\def\iisf{{\sf ii}}
\def\iiisf{{\sf iii}}
\def\jsf{{\sf j}}
\def\ksf{{\sf k}}
\def\lsf{{\sf l}}
\def\ellsf{{\sf \ell}}
\def\msf{{\sf m}}
\def\nsf{{\sf n}}
\def\osf{{\sf o}}
\def\psf{{\sf p}}
\def\qsf{{\sf q}}
\def\rsf{{\sf r}}
\def\ssf{{\sf s}}
\def\tsf{{\sf t}}
\def\usf{{\sf u}}
\def\vsf{{\sf v}}
\def\wsf{{\sf w}}
\def\xsf{{\sf x}}
\def\ysf{{\sf y}}
\def\zsf{{\sf z}}
\def\rsf{{\sf r}}
\def\xsf{{\sf x}}
\def\ysf{{\sf y}}
\def\Asf{{\sf A}}
\def\Bsf{{\sf B}}
\def\Csf{{\sf C}}
\def\Dsf{{\sf D}}
\def\Esf{{\sf E}}
\def\Fsf{{\sf F}}
\def\Gsf{{\sf G}}
\def\Hsf{{\sf H}}
\def\Isf{{\sf I}}
\def\Jsf{{\sf J}}
\def\Ksf{{\sf K}}
\def\Lsf{{\sf L}}
\def\Msf{{\sf M}}
\def\Nsf{{\sf N}}
\def\Osf{{\sf O}}
\def\Psf{{\sf P}}
\def\Qsf{{\sf Q}}
\def\Rsf{{\sf R}}
\def\Ssf{{\sf S}}
\def\Tsf{{\sf T}}
\def\Usf{{\sf U}}
\def\Vsf{{\sf V}}
\def\Wsf{{\sf W}}
\def\Xsf{{\sf X}}
\def\Ysf{{\sf Y}}
\def\Zsf{{\sf Z}}
\def\CRB{{\bf CRB}}
\def\FIM{{\bf FIM}}
\def\Ac{{\cal A}}
\def\Bc{{\cal B}}
\def\Cc{{\cal C}}
\def\Dc{{\cal D}}
\def\Ec{{\cal E}}
\def\Fc{{\cal F}}
\def\Gc{{\cal G}}
\def\Hc{{\cal H}}
\def\Ic{{\cal I}}
\def\Jc{{\cal J}}
\def\Kc{{\cal K}}
\def\Lc{{\cal L}}
\def\Mc{{\cal M}}
\def\Nc{{\cal N}}
\def\Oc{{\cal O}}
\def\Pc{{\cal P}}
\def\Qc{{\cal Q}}
\def\Rc{{\cal R}}
\def\Sc{{\cal S}}
\def\Tc{{\cal T}}
\def\Uc{{\cal U}}
\def\Vc{{\cal V}}
\def\Wc{{\cal W}}
\def\Xc{{\cal X}}
\def\Yc{{\cal Y}}
\def\Zc{{\cal Z}}
\def\xbfhat{\hat{\xbf}}
\def\lambdahat{\hat{\lambda}}
\def\lh{\hat{\lambda}}
\def\dh{\hat{d}}
\def\sh{\hat{s}}
\def\sdhh{\hat{\hat{s}}_d}
\def\wh{\hat{\wbf}}
\def\Phibar{\bar{\Phibf}}
\def\lambdatilde{\tilde{\lambda}}
\def\lambdabfhat{\hat{\lambdabf}}
\def\lambdatbf{{\tilde {\lambdabf}}}
\def\At{{\tilde{\Abf}}}
\def\Bt{{\tilde{\Bbf}}}
\def\Ath{{\hat{\tilde{\Abf}}}}
\def\Gt{{\tilde{\Gbf}}}
\def\Tt{{\tilde{\T}}}
\def\Ah{{\hat{\Abf}}}
\def\Gh{{\hat{\Gbf}}}
\def\Qh{{\hat{\Qbf}}}
\def\Th{{\hat{\T}}}
\def\Uh{{\hat{\U}}}
\def\a{{\abf}}
\def\d{{\dbf}}
\def\s{{\sbf}}
\def\x{{\xbf}}
\def\y{{\ybf}}
\def\at{{\tilde{\abf}}}
\def\bt{{\tilde{\bbf}}}
\def\ah{{\hat{\abf}}}
\def\th{{\theta}}
\def\thh{{\hat{\theta}}}
\def\thi{{\theta_i}}
\def\thih{{\hat{\theta}_i}}
\def\thk{{\theta_k}}
\def\thik{{\hat{\theta}_k}}
\def\ai{{\a(\theta_i)}}
\def\ath{{\a(\theta)}}
\def\aths{{\a^*(\theta)}}
\def\athT{{\a^T(\theta)}}
\def\ais{{\a^*(\theta_i)}}
\def\ait{{\a^T(\theta_i)}}
\def\ak{{\a(\theta_k)}}
\def\aks{{\a^*(\theta_k)}}
\def\akt{{\a^T(\theta_k)}}
\def\thbf{{\thetabf}}
\def\sbft{{\tilde{\sbf}}}
\def\thbft{{\tilde{\thbf}}}
\def\thbfh{{\hat{\thbf}}}
\def\rhobfh{{\hat{\rhobf}}}
\def\thbfhh{{\hat{\hat{\thbf}}}}
\def\etat{{\tilde{\eta}}}
\def\etabft{{\tilde{\etabf}}}
\def\etabfth{{\hat{\tilde{\etabf}}}}
\def\etabfhh{{\hat{\hat{\etabf}}}}
\def\etabfh{{\hat{\etabf}}}
\def\alphabfh{{\hat{\alphabf}}}
\def\Vh{{\hat{V}}}
\def\Vt{{\tilde{V}}}
\def\therr{{\hat{\theta}-\theta}}
\def\therrbf{{\hat{\thetabf}-\thetabf_0}}
\def\therrbfwsf{{\hat{\thetabf}_\WSF-\thetabf_0}}
\def\etaerr{{\hat{\eta}-\eta}}
\def\etaerrbf{{\hat{\etabf}-\etabf_0}}
\def\etabfhat{{\hat{\etabf}}}
\def\ebh{{\etabfhat}}
\def\ebz{{\etabf_0}}
\def\Capo{{\C^{pq}_{a,1}}}
\def\Capt{{\C^{pq}_{a,2}}}
\def\Cesp{{\C_\ES}}
\def\therri{{\thih-\thi}}
\def\therrk{{\thik-\thk}}
\def\Cxik{{\Cbf_{\xi,1}^{ik}}}
\def\CxikT{{\Cbf_{\xi,2}^{ik}}}
\def\Cxpq{{\Cbf_{\xi,1}^{pq}}}
\def\CxpqT{{\Cbf_{\xi,2}^{pq}}}
\def\Cxii{{\Cbf_{\xi,1}^{ii}}}
\def\CxiiT{{\Cbf_{\xi,2}^{ii}}}
\def\Cxi{{\Cbf_{\xi,1}^{i}}}
\def\CxiT{{\Cbf_{\xi,2}^{i}}}
\def\Cx{{\Cbf_{\xi,1}}}
\def\CxT{{\Cbf_{\xi,2}}}
\def\Cmu{{\Cbf_{\MU}}}
\def\Cmuf{{\Cbf_{\MUF}}}
\def\Cmuik{{\Cbf_{\MU,ik}}}
\def\Cwmu{{\Cbf_{\WMU}}}
\def\Cwmuik{{\Cbf_{\WMU,ik}}}
\def\Lsl{{\Lambdabf_s}}
\def\Ls{{\Lambdabf_s}}
\def\Lh{{\hat{\Lambdabf}}}
%\def\Lsh{{\hat{\Lambdabf}_s}}
\def\Lshat{{\Lsh}}
\def\Lnh{{\hat{\Lambdabf}_n}}
\def\Lnhi{{\hat{\Lambdabf}_n^{-1}}}
\def\Lst{{\tilde{\Lambdabf}_s}}
\def\Lnt{{\tilde{\Lambdabf}_n}}
\def\Lt{{\tilde{\Lambdabf}}}
\def\Ltilde{{\Lt}}
\def\Lo{{\overline{\Lambdabf}}}
\def\Cx{{\Cbf_{\xi,1}}}
\def\CxT{{\Cbf_{\xi,2}}}
\def\pht{{\tilde{\phi}}}
\def\gt{{\tilde{g}}}
\def\xt{{\tilde{x}}}
\def\yt{{\tilde{y}}}
\def\xbft{{\tilde{\xbf}}}
\def\ybft{{\tilde{\ybf}}}
\def\gtogk{{{\gt_k}\over{g_k}}}
\def\atoak{{{\tilde{a}_k}\over{a_k}}}
\def\w{{\omega}}
\def\EEP{{\Ebar_W^*\Ebar_W \Pbf_{\bar{\Psibf}^*}^\perp}}
\def\EPp{{\Ebar_W \P_{\bar{\Psibf}^*}^\perp}}
\def\EP{{\Ebar_W \P_{\bar{\Psibf}^*}}}
\def\Eyha{{{\hat{\Ebf}}_y^\phstar}}
\def\LPbar{{\Psibar^*(\Psibar\Psibar^*)^{-1}}}
\def\PPbar{{\Psibar^*(\Psibar\Psibar^*)^{-1}\Psibar}}
\def\ppij{{{\partial}\over{\Psibf_{ij}}}}
\def\Pho{{{\hat{\Psibf}}_1}}
\def\Phw{{{\hat{\Psibf}}_2}}
\def\Phh{{{\hat{\Psibf}}_3}}
\def\pho{{{\hat{\psibf}}_1}}
\def\phw{{{\hat{\psibf}}_2}}
\def\phh{{{\hat{\psibf}}_3}}
\def\Pbh{{{\hat{\Psibar}}}}
\def\Pti{{{\tilde{\Psibf}}_i}}
\def\Pbi{{{\hat{\Psibf}}_i}}
\def\pto{{{\tilde{\psibf}}_1}}
\def\ptw{{{\tilde{\psibf}}_2}}
\def\pth{{{\tilde{\psibf}}_3}}
\def\Pto{{{\tilde{\Psibf}}_1}}
\def\Ptw{{{\tilde{\Psibf}}_2}}
\def\Pth{{{\tilde{\Psibf}}_3}}
\def\Pbt{{{\tilde{\Psibar}}}}
\def\En{{\Ebf_n}}
\def\Es{{\Ebf_s}}
\def\Ens{{\Ebf_n^*}}
\def\Ess{{\Ebf_s^*}}
\def\Eh{{\hat{\E}}}
\def\Et{{\tilde{\E}}}
\def\Ehh{{\hat{\hat{\E}}}}
\def\Ett{{\tilde{\tilde{\E}}}}
\def\Eshh{{\hat{\hat{\Ebf}}_s}}
\def\Enhh{{\hat{\hat{\Ebf}}_n}}
\def\Eshhs{{\hat{\hat{\Ebf}}_s^*}}
\def\Enhhs{{\hat{\hat{\Ebf}}_n^*}}
\def\Ent{{{\tilde{\Ebf}}_n}}
\def\Est{{{\tilde{\Ebf}}_s}}
\def\Entt{{\tilde{\tilde{\Ebf}}_n}}
\def\Estt{{\tilde{\tilde{\Ebf}}_s}}
\def\Entts{{\tilde{\tilde{\Ebf}}_n^*}}
\def\Estts{{\tilde{\tilde{\Ebf}}_s^*}}
\def\Ents{{{\tilde{\Ebf}}_n^*}}
\def\Ests{{{\tilde{\Ebf}}_s^*}}
\def\Enh{{\hat{\Ebf}_n}}
\def\Esh{{\hat{\Ebf}_s}}
\def\Enhs{{\hat{\Ebf}_n^*}}
\def\Eshs{{\hat{\Ebf}_s^*}}
\def\Eshz{{\hat{\Ebf}_0}}
\def\Esho{{\hat{\Ebf}_1}}
\def\Eshp{{\hat{\Ebf}_{p-1}}}
\def\EEs{{\Ebf_s^{}\Ebf_s^*}}
\def\EEsh{{\hat{\Ebf}_s^{}\hat{\Ebf}_s^*}}
\def\EEn{{\Ebf_n^{}\Ebf_n^*}}
\def\EEnh{{\hat{\Ebf}_n^{}\hat{\Ebf}_n^*}}
\newcommand{\ENEN}{\mbox{$\hat{\Ebf}_n^{}\hat{\Ebf}_n^*$}}
\def\EWE{{\Ebf_s^{}\Wbf\Ebf_s^*}}
\def\EWEh{{\hat{\Ebf}_s^{}\Wbf\hat{\Ebf}_s^*}}
\def\EWsEh{{\hat{\Ebf}_s^{}\Wbf_s^{}\hat{\Ebf}_s^*}}
\def\EWchEh{{\hat{\Ebf}_s^{}\hat{\Wbf}_c^{}\hat{\Ebf}_s^*}}
\def\EWot{{\Ebf_s \Wbf^{\half}}}
\def\EWoth{{\hat{\Ebf}_s^{} \Wbf^{\half}}}
\def\EWchoth{{\hat{\Ebf}_s^{} \hat{\Wbf}_c^{\half}}}
\def\et{{\tilde{\ebf}}}
\def\eh{{\hat{\ebf}}}
\def\ett{{\tilde{\tilde{\ebf}}}}
\def\ehh{{\hat{\hat{\ebf}}}}
\def\Wcot{{\Wbf_c^{\half}}}
\def\Wrot{{\Wbf_r^{\half}}}
\def\Deltaeq{{\stackrel{\Delta}{=}}}
\def\A{{\Abf}}
\def\B{{\Bbf}}
\def\C{{\Cbf}}
\def\D{{\Dbf}}
\def\E{{\Ebf}}
\def\F{{\Fbf}}
\def\G{{\Gbf}}
\def\H{{\Hbf}}
\def\I{{\Ibf}}
\def\It{{\tilde{\Ibf}}}
\def\J{{\Jbf}}
\def\K{{\Kbf}}
\def\L{{\Lbf}}
\def\M{{\Mbf}}
\def\N{{\Nbf}}
\def\P{{\Pbf}}
\def\Q{{\Qbf}}
\def\R{{\Rbf}}
\def\S{{\Sbf}}
\def\T{{\Tbf}}
\def\U{{\Ubf}}
\def\V{{\Vbf}}
\def\W{{\Wbf}}
\def\X{{\Xbf}}
\def\Y{{\Ybf}}
\def\Z{{\Zbf}}
\def\SNR{{\mbox{\rm SNR}}}
\def\ssSigma{{\scriptscriptstyle \Sigma}}
\def\CB{{\scriptscriptstyle CB}}
\def\CML{{\scriptscriptstyle CML}}
\def\UML{{\scriptscriptstyle UML}}
\def\DML{{\scriptscriptstyle DML}}
\def\SML{{\scriptscriptstyle SML}}
\def\ML{{\scriptscriptstyle ML}}
\def\MD{{\scriptscriptstyle MD}}
\def\MU{{\scriptscriptstyle MU}}
\def\MUF{{\scriptscriptstyle MUF}}
\def\MUD{{\scriptscriptstyle MUD}}
\def\MUDc{{\scriptscriptstyle MUDc}}
\def\WMU{{\scriptscriptstyle WMU}}
\def\MO{{\scriptscriptstyle MO}}
\def\ES{{\scriptscriptstyle ES}}
\def\MSE{{\scriptscriptstyle MSE}}
\def\LS{{\scriptscriptstyle LS}}
\def\TLS{{\scriptscriptstyle TLS}}
\def\BF{{\scriptscriptstyle BF}}
\def\FS{{\scriptscriptstyle FS}}
\def\AR{{\scriptscriptstyle AR}}
\def\WSF{{\scriptscriptstyle WSF}}
\def\OSF{{\scriptscriptstyle OSF}}
\def\SSF{{\scriptscriptstyle SSF}}
\def\RSF{{\scriptscriptstyle RSF}}
\def\NSF{{\scriptscriptstyle NSF}}
\def\MAP{{\scriptscriptstyle MAP}}
\def\OPT{{\scriptscriptstyle OPT}}
\def\FA{{\scriptscriptstyle FA}}
\def\SSE{{\scriptscriptstyle SSE}}
\def\LCMV{{\scriptscriptstyle LCMV}}
\def\SC{{\scriptscriptstyle SC}}
\def\WLS{{\scriptscriptstyle WLS}}
\def\aQa{{\abf^*\Qbf^{-1}\abf}}
\def\dQa{{\dbf^*\Qbf^{-1}\abf}}
\def\aQd{{\abf^*\Qbf^{-1}\dbf}}
\def\dQd{{\dbf^*\Qbf^{-1}\dbf}}
\def\zerobf{{\bf 0}}
\def\onebf{{\bf 1}}
\def\half{{{1}\over{2}}}
\def\halfT{{{*}\over{2}}}
\def\jhalf{{{j}\over{2}}}
\def\mjhalf{{{-j}\over{2}}}
\def\mhalf{{-\half}}
\def\Rss{{\Rbf_{ss}}}
\def\Rssi{{\Rbf_{ss}^{-1}}}
\def\Rsst{{\R_{\sbf\tilde{s}}}}
\def\RsstH{{\R_{\sbf\tilde{s}}^*}}
\def\Rssb{{\Rbf_{\sbf\sbf}}}
\def\Rssbi{{\Rbf_{\sbf\sbf}^{-1}}}
\def\Rssd{{\Rbf_{\sbf s_d}}}
\def\RssdH{{\Rbf_{\sbf s_d}^*}}
\def\Rssh{{\hat{\Rbf}_{ss}}}
\def\Rxs{{\Rbf_{xs}}}
\def\Rxsb{{\Rbf_{\xbf\sbf}}}
\def\RxsH{{\Rbf_{x\sh}}}
\def\Rxx{{\Rbf_{xx}}}
\def\Rxxb{{\Rbf_{\xbf\xbf}}}
\def\Rxxbi{{\Rbf_{\xbf\xbf}^{-1}}}
\def\Rxxh{{\hat{\Rbf}_{xx}}}
\def\Ryyh{{\hat{\Rbf}_{yy}}}
\def\Rysh{{\hat{\Rbf}_{ys}}}
\def\Rxxo{{\Rbf_{xx0}}}
\def\Rzz{{\Rbf_{zz}}}
\def\Rzzh{{\hat{\Rbf}_{zz}}}
\def\Rh{{\hat{\R}}}
\def\Rhi{{\hat{\R}^{-1}}}
\def\Rhat{{\Rh}}
\def\Sh{{\hat{\S}}}
\def\St{{\tilde{\S}}}
\def\Xh{{\hat{\X}}}
\def\Xt{{\tilde{\X}}}
\def\Ad{{\A^\dag}}
\def\Adt{{\A^{\dag *}}}
\def\Sd{{\S^\dag}}
\def\Sdt{{\S^{\dag *}}}
\def\Th{{\hat{\T}}}
\def\Wh{{\hat{\W}}}
\def\Wt{{\tilde{\W}}}
\def\Rt{{\tilde{\R}}}
\def\Rhs{{\Rh^{}_\Sigma}}
%%\def\Rs{{\R^{}_\Sigma}}
\def\PAp{{\P_A^\perp}}
\def\PA0p{{\P_{A_0}^\perp}}
\def\PAs{{\P^{}_{{\Sigma^\mhalf A}}}}
\def\PAps{{\P^\perp_{{\Sigma^\mhalf A}}}}
\def\Pas{{\P^{}_{{\Sigma^\mhalf a(\theta)}}}}
\def\Paps{{\P^\perp_{{\Sigma^\mhalf a(\theta)}}}}
\def\DA{{\Delta\A}}
\def\Dt{{\Deltabf}}
\def\Sgbf{{\Sigmabf}}
\def\Sgbfh{{\hat{\Sigmabf}}}
\def\Sgbft{{\tilde{\Sgbf}}}
\def\Sgot{{\Sgbf^\mhalf}}
\def\Sgotm{{\Sgbf^\half}}
\def\Sgi{{\Sgbf^{-1}}}
\def\sg{{\sigma}}
\def\snt{{\sigma_n^2}}
\def\sdt{{\sigma_d^2}}
\def\snth{{\hat{\sigma}_n^2}}
\def\sat{{\sigma_a^2}}
\def\stwo{{\sigma^2}}
\def\s2h{{\hat{\sigma}^2}}
\def\Trss{{\Tr(\Rss)}}
\def\real{{\mbox{\rm real}}}
\def\imag{{\mbox{\rm imag}}}
\def\diag{{\mbox{\rm diag}}}
\def\spann{{\mbox{\rm span}}}
\def\Re{{\mbox{\rm Re}}}
\def\Im{{\mbox{\rm Im}}}
\def\Tr{{\mbox{\rm Tr}}}
\def\vecc{{\mbox{\rm vec}}}
\def\det{{\mbox{\rm det}}}
\def\rank{{\mbox{\rm rank}}}
\def\ba{\begin{array}}
\def\ea{\end{array}}
\def\bea{\begin{eqnarray}}
\def\eea{\end{eqnarray}}
\def\beas{\begin{eqnarray*}}
\def\eeas{\end{eqnarray*}}
\newcommand{\onempphp}[1]{
  \iftwocol  \unitlength .45pt
    \[\begin{picture}(440,320)(0,0)
     \special{psfile=#1 hscale=45 vscale=45 voffset=-10}%
    \end{picture}\]
  \else  \unitlength .8pt
    \begin{center} \begin{picture}(440,290)(0,0)
     \special{psfile=#1 hscale=.90 vscale=.80 hoffset=-20 voffset=-25}%
    \end{picture} \end{center}
  \fi
}

% Local Variables:
% mode: plain-tex
% TeX-master: t
% End:

